A month of monitoring the new magnetar Swift J1555.2-5402 during an X-ray outburst

The soft gamma-ray repeater Swift J1555.2-5402 was discovered by means of a 12-ms duration short burst detected with Swift BAT on 2021 June 3. Then 1.6 hours after the first burst detection, NICER started daily monitoring of this X-ray source for a month. The absorbed 2-10 keV flux stays nearly constant at around 4e-11 erg/s/cm2 during the monitoring timespan, showing only a slight gradual decline. A 3.86-s periodicity is detected, and the time derivative of this period is measured to be 3.05(7)e-11 s/s. The soft X-ray pulse shows a single sinusoidal shape with a root-mean-square pulsed fraction that increases as a function of energy from 15% at 1.5 keV to 39% at 7 keV. The equatorial surface magnetic field, characteristic age, and spin-down luminosity are derived under the dipole field approximation to be 3.5e+14 G, 2.0 kyr, and 2.1e+34 erg/s, respectively. An absorbed blackbody with a temperature of 1.1 keV approximates the soft X-ray spectrum. Assuming a source distance of 10 kpc, the peak X-ray luminosity is ~8.5e+35 erg/s in the 2--10 keV band. During the period of observations, we detect 5 and 37 short bursts with Swift/BAT and NICER, respectively. Based on these observational properties, especially the inferred strong magnetic field, this new source is classified as a magnetar. We also coordinated hard X-ray and radio observations with NuSTAR, DSN, and VERA. A hard X-ray power-law component that extends up to at least 40 keV is detected at 3-sigma significance. The 10-60 keV flux, which is dominated by the power-law component, is ~9e-12 erg/s/cm2 with a photon index of ~1.2. The pulsed fraction has a sharp cutoff above 10 keV, down to ~10% in the hard-tail component band. No radio pulsations are detected during the DSN nor VERA observations. We place 7{\sigma} upper limits of 0.043mJy and 0.026 mJy on the flux density at S-band and X-band, respectively.

==> tab_glitch_seg.tex <==
\begin{deluxetable*}{lrrr}
%\tablenum{1}
\tablecaption{Summary of the glitch model for \src \label{tab:summary_glitch}}
\tablewidth{0pt}
\tablehead{
\colhead{Parameter} & \multicolumn{3}{c}{Values} 
}
%\decimalcolnumbers
\startdata
Glitch Candidate & 1 & 2 & 3 \\ 
\hline
MJD range & 59368.5298--59379.8664 & 59380.6386--59387.4267 & 59388.2551--59396.9801 \\
Epoch $T_0$ (MJD) & 59374.1981 & 59384.0326 & 59392.6176 \\
Glitch Epoch (MJD) & 59373.6412 & 59382.9236 & 59394.0398 \\
Spin frequency $\nu$ (Hz) & 0.25899847(5) & 0.2589973(7) & 0.2590474(14) \\
Frequency derivative $\dot{\nu}$ (Hz~s$^{-1}$) & $-1.63(19)\times 10^{-12}$ & $4(37)\times 10^{-13}$ & $1.56(4)\times10^{-10}$ \\
$\Delta\nu$ (Hz) & $-3.6(7)\times10^{-5}$ & $-0.2(5.3)\times10^{-7}$ & $-2.14(6)\times10^{-5}$ \\
$\Delta\dot{\nu}$ (Hz~s$^{-1}$) & $3.4(2.1)\times10^{-13}$ & $-4.4(3.4)\times10^{-12}$ & $-1.46(4)\times10^{-10}$ \\
RMS residual (phase) & 0.012 & 0.017 & 0.040 \\
$\chi^2$/d.o.f. & 79.344/72 & 22.884/29 & 97.894/15 \\
\hline 
$\Delta\nu/\nu$ & $-1.4(0.3)\times10^{-6}$ & $-0.08(205)\times10^{-8}$ & $-8.3(2)\times10^{-5}$ \\
$\Delta\dot{\nu}/\dot{\nu}$ & -0.21(13) & -11(102) & -0.94(4) \\
\enddata 
\end{deluxetable*}

%Glitch 1: Delta nu/nu = -1.3787074532062746e-06 +- 2.8862253058150074e-07
%Glitch 1: Delta nudot/nudot = -0.20724605309569824 +- 0.12914793749632392
%Glitch 2: Delta nu/nu = -7.944888620179421e-08 +- 2.0467724493379157e-06
%Glitch 2: Delta nudot/nudot = -11.027715443558105 +- 102.08166205820072
%Glitch 3: Delta nu/nu = -8.269565200820224e-05 +- 2.28295336192605e-06
%Glitch 3: Delta nudot/nudot = -0.9382721139426152 +- 0.036751685876285196
